Bridging Model Heterogeneity in Federated Learning via Uncertainty-based Asymmetrical Reciprocity Learning

This paper presents FedType, a simple yet pioneering framework designed to fill research gaps in heterogeneous model aggregation within federated learning (FL). FedType introduces small identical proxy models for clients, serving as agents for information exchange, ensuring model security, and achieving efficient communication simultaneously. To transfer knowledge between large private and small proxy models on clients, we propose a novel uncertainty-based asymmetrical reciprocity learning method, eliminating the need for any public data. Comprehensive experiments conducted on benchmark datasets demonstrate the efficacy and generalization ability of FedType across diverse settings. Our approach redefines federated learning paradigms by bridging model heterogeneity, eliminating reliance on public data, prioritizing client privacy, and reducing communication costs.

==> section/insight.tex <==
\section{Model Insight}
\subsection{Core Model Capability Study}
In this subsection, we study the effect on the performance brought by the proxy model selection.  We test extra four classical models including MobileNetV1~\cite{howard2017mobilenets}, GoogLeNet~\cite{szegedy2015going}, EfficientnetB0~\cite{tan2019efficientnet}, 

we cite this \hyperlink{1}{https://paperswithcode.com/sota/image-classification-on-cifar-10?p=efficientnetv2-smaller-models-and-faster} and \hyperlink{2}{https://github.com/JustinYuu/pytorch-CIFAR10-playground}

\subsection{Convergence Analysis}
Optional, show with figures
\subsection{$g$ Function Study}
We conduct a study on the different selections of $\lambda$ functions including the linear function, quadratic function, and Sigmoid function when  $\Delta^t < 0$. In our experiment, we set $\lambda = 0.5$. There are some basic requirements they are designed to meet: (1) when $\Delta^t=0$, $g(\Delta^t, \lambda) = 0.5$, (2) when $\Delta^t=-1$, $g(\Delta^t, \lambda)$ is is approach 1 or equal to 1. 
\begin{itemize}
    \item Linear:$g(\Delta^t, \lambda) =  0.5 $ (results obtained from ablation study)
    \item Linear:$g(\Delta^t, \lambda) =  -0.5 \times \Delta^t +0.5 $ (results in table 1)
    \item Quadratic: $g(\Delta^t, \lambda) = 0.5 \times {\Delta^t}^{2} + 0.5$
    \item Sigmoid: $g(\Delta^t, \lambda) =2.164\times 1/(1+e^{ \Delta^t})-0.582$
\end{itemize}

\begin{table}[h!]
\centering
\caption{$\lambda$ function study, Cifar10}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc} 
\toprule 
\textbf{Dataset}& \multicolumn{3}{c|}{\textbf{1}}&
\multicolumn{3}{c|}{\textbf{0.5}} & \multicolumn{3}{c}{\textbf{0.1}}\\
% \textbf{Option} & $10\%$ & $20\%$ & $ 30\%$ & $10\%$ & $20\%$ & $ 30\%$& $10\%$ & $20\%$ & $ 30\%$\\
\midrule
Linear   \\ 
Quadratic \\
Sigmoid\\
\bottomrule 
\end{tabular}
}
\label{tab:lambda}
\end{table}



\subsection{Scalability Test}

\begin{table}[ht]
\centering
\caption{Scale, cross-device, 50, 100, 150 are the client number, 10\%,20\%,30\% are the sample ratio, we use CIFAR-10 as the data.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccc} 
\toprule 
\textbf{Setting}  & 50& 100 &150\\
\midrule
10\%   \\ 
20\%\\
30\% \\
\bottomrule 
\end{tabular}
}
\label{tab:scale}
\end{table}
\subsection{Knowledge Transfer Analysis}


==> section/method.tex <==

\clearpage
\newpage
\section{Methodology}
\begin{figure*}[t!]
\centering
\includegraphics[width=0.88\textwidth]{figure/framework_placeholder.pdf}
    % \vspace{-0.1in}
    \caption{Overview of the proposed \ours framework.\textcolor{blue}{placeholder}}
    \label{fig:overview}
    % \vspace{-0.1in}
\end{figure*}
\subsection{Overview}
The goal of this work is to design a unified federated learning framework which breaks the model structure barrier and can be generally applied in different scenarios. Let $\mathcal{D}_i = \{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{|\mathcal{D}_n|}$ denote the training data stored in the $n$-th local client $L_n$, where $\mathbf{x}_i$ denotes the data, $\mathbf{y}_i$ is the ground truth label, and $|\mathcal{D}_i|$ is the number of training data. Each client owns one private model $\mathbf{w}_i$ and a proxy model $\overline{{\mathbf{w}_i}}$ to train its training data. Note that the client models $\{\mathbf{w}_1, \cdots, \mathbf{w}_N\}$ do not have to share identical network structures, where $N$ is the total number of clients. The overview of our framework is shown in Figure. At communication round $t$, $B$ ($B\le N$) clients are selected to participate in the update process. First, each selected client $i$ ($n\in B$) will generate a proxy and compact model $\overline{{\mathbf{w}_i^t}}$ using the local data $\mathcal{D}_i$ with the help of its private model $\mathbf{w}_i^t$. Second, the selected clients upload the proxy and compact models $\overline{{\mathbf{w}_1^t}}, \overline{{\mathbf{w}_1^t}}, \cdot, \overline{{\mathbf{w}_B^t}}$ to the server. Second, the server aggregates the received models to $\overline{{\mathbf{w}_G^t}}$ and distributes it back to the clients. Third, after receiving the aggregated model, the selected clients will conduct the asymmetric reciprocal learning to update the proxy model and the private model simultaneously with the local data. Next, we provide the details of the designed algorithm.

\subsection{Asymmetric Reciprocal Learning}
Each client $i$ holds a model $\mathbf{w}_i^t$ at communication round $t$.The traditional FedAvg-based method typically involves uploading the client's model to a server for aggregation. However, this approach presents two significant concerns: (1) In many real-world applications, particularly in sensitive areas like healthcare and finance, there are stringent restrictions against sharing private model structures and parameters trained on confidential data. (2) The transmission of large models entails substantial communication costs, which can result in significant latency issues. To address these challenges, our approach involves developing a compact and proxy model derived from the private model. This proxy model, rather than the original, is transmitted over the network for each client, effectively navigating the aforementioned issues.

A straightforward approach would be to use the large model $\mathbf{w}_i$ as a 'teacher' and apply knowledge distillation on local data $\mathcal{D}_i$ to derive a smaller, compact proxy model. These proxy models would then be the ones exchanged between the server and clients. However, this method overlooks the substantial disparity in information content and modeling capacity between the large private model $\mathbf{w}_i$ and its compact counterpart $\overline{\mathbf{w}_i}$. Firstly, when proxy models are aggregated on the server, the refined proxy model gains diverse and essential insights from other participating clients. Secondly, there's an inherent difference in capability due to the size variance; the larger private model $\mathbf{w}_i$ inherently possesses greater computational power than the smaller proxy model $\overline{\mathbf{w}_i}$. This discrepancy leads to a critical and challenging research question: \emph{How can we devise a learning mechanism that allows both the large private model and the smaller proxy model to mutually benefit, considering their differing capabilities and the diversity of information each model contains?}

To track this issue, we propose a novel asymmetric reciprocal learning (\texttt{ARL}) strategy to update the private model and proxy model \emph{simultaneously} and \emph{alternately}. Specifically, the designed \texttt{ARL} strategy covers the two parts including \textbf{proxy model forward coaching} and \textbf{private model backward feeding}, which enables the knowledge to transfer between the two models in a bi-directional way. We will introduce the two steps in detail as follows.

\subsection{Proxy Model Forward Coaching}
In the proxy model forward coaching process, we expect the large private model to transfer the knowledge to the small proxy model and the proxy model is able to imitate the behaviors of the private model. Thus, we treat the private model $\mathbf{w}_i$ as the teacher and the proxy model $\overline{{\mathbf{w}_i}}$ as the student:

\begin{equation}\label{eq:proxy_model}
    \overline{\mathcal{L}_i} = \sum_{k=1}^{K_i}\text{KL}(\mathbf{w}_i(\mathbf{x}^{i}_k) || \overline{\mathbf{w}}_i(\mathbf{x}^{i}_k)),
\end{equation}
where $\mathbf{x}^{i}_k$ is the $k^{th}$ data, and ${K_i}$ is total number of $\mathcal{D}_j^l$, KL is Kullback–Leibler divergence. 

\subsection{Private Model Backward Feeding}
Generally speaking, the private models are usually more powerful than the compact proxy models considering the different model sizes. If directly conduct the same approach to transfer knowledge from the proxy model to the private model, considering the credibility of the two models, it may not be guaranteed that the large model will get boosted due to the potential noise caused by the proxy model. 

To address this issue, we introduce a \emph{certainty-based backward feeding} strategy. This method does not indiscriminately back-feed all class knowledge from the dataset to the private model. Instead, it selectively back-feeds only those classes $\Omega_i$ for which the private model demonstrates higher confidence in its output for client $i$. Additionally, we anticipate that the large model can more effectively discern selected classes under a less stringent framework, as opposed to the rigorous knowledge distillation process for each individual logit. Therefore, we suggest a certainty-based knowledge distillation approach, denoted as \texttt{CKD}, which enables the large model to mimic the proxy model's behaviors within a specified range. Specifically, we enforce to improve the ranks of these top classes in $\overline{\mathbf{w}_i(\mathbf{x}_{k}^{i})}$ using the following loss:
\begin{equation}\label{eq:certainty_KD}
\begin{split}
    &\overleftarrow{\mathcal{KD}_i} = \sum_{k=1}^{K_i} \sum_{r \in \overline{\Omega}} \log(\frac{\exp(\mathbf{w}_i(\mathbf{x}_{k}^{i})[r])}{\Phi}),\\
    \Phi = &\sum_{u \in \overline{\Omega}} \exp(\mathbf{w}_i(\mathbf{x}_{k}^{i})[u]) + \sum_{v \in \overline{\Omega^\prime}} \exp(\mathbf{w}_i(\mathbf{x}_{k}^{i})[v]),
\end{split}
\end{equation}

where $\overline{\Omega}$ denotes the high-certainty class index set, $\overline{\Omega^\prime}$ represents the set cosisting of remaining classes, and $\beta$ is the weighted hyperparameter. The primary role of Eq.~\eqref{eq:certainty_KD} is to utilize the top class ranks $\overline{\Omega}$, as determined by the proxy model, to guide and enhance the accuracy of the corresponding class probabilities in the larger model. This approach eases the stringent demands of traditional knowledge distillation, allowing the larger model to more fluidly emulate the proxy model's behavior. So far, combined with the the classical training process, the update of the private model can be formulated as:

\begin{equation}\label{eq:private_model}
   \mathcal{L}_{i} = \text{CE}(\mathbf{w}_i(\mathbf{x}_i), \mathbf{y}_i) + \beta_i \cdot \overleftarrow{\mathcal{KD}}_i
\end{equation}


Nevertheless, this method introduces two additional complexities: (1) Generating the high-certain class index set $\overline{\Omega}$ is non-trivial. Simply setting a fixed parameter $\nu$ to select the classes with top-$\nu$ largest logits may not be effective due to the continuous learning process and the iterative update nature of federated learning. (2) The choice of the hyperparameter $\beta$ is pivotal, as it regulates the extent of information fed back to the larger model by adjusting the loss weight during optimization. Determining its value accurately amidst dynamic updates presents a significant challenge. To address these issues, we propose two distinct strategies for determining the optimal top-ranked class set $\Omega$ and the appropriate weighting of the hyperparameter $\beta$.

\noindent\textbf{Certainty-based Class Selection}
To appropriately identify the target class set, we consider the certainty of the proxy model $\overline{{\mathbf{w}_i}}$ on the input data $\mathbf{x}^{k}_{i}$. Here, we leverage the conformal calibration ~\cite{gupta2022nested,angelopoulos2020uncertainty} to identify the valid high-certainty prediction sets for the private model and the proxy model. Specifically, given the input data $\mathbf{x}_{i}$ and the model $w_i$ at each client $i$, we construct :

\begin{equation}\label{eq:conformal}
\small{
\begin{split}
    \overline{\Omega_i} (\mathbf{x}_{i})&\rightarrow \left\{ \mathbf{w}_i(\mathbf{x}^{i}
    ) : \rho_{x}(\overline{\mathbf{w}_i}(\mathbf{x}_{i}
    )) + \hat{\pi} (\overline{\mathbf{w}_i}(\mathbf{x}_{i}
    )) \cdot u   +  \mathcal{R}\right\}\\
    \mathcal{R} &= \lambda \cdot (o_{x_{i}}(\overline{\mathbf{w}_i}(\mathbf{x}_{i}
    ))-k_{reg}^{+} \leq \tau),
\end{split}}
\end{equation}
where $\overline{\mathbf{w}_i}(\mathbf{x}^{i})$ is the output of the model, $\rho_{x}(\overline{\mathbf{w}_i}(\mathbf{x}^{i}))$ is the total probability mass of the set of labels that are more likely than the output of the model, $\hat{\pi} (\overline{\mathbf{w}_i}(\mathbf{x}^{i}
    ))$ is the computed class probabilities, $\mathcal{R}$ is the regularization, $\lambda$ and $k_{reg}$ are the hyperparameters to control the set size.

Now, given the proxy model $\overline{{\mathbf{w}_i}}$ and the input data $x_i$ using the conformal prediction approach, we are able to obtain the prediction set $\overline{\Omega_i}$ with high certainty, which contains $V$ labels. Till now, we have successfully identified the high-certainty labels predicted by the proxy model $\overline{{\mathbf{w}_i}}$ for client $i$. 

\noindent\textbf{Consensus-based Bi-optimization} In this subsection, we introduce how to obtain the hyperparameter $\beta$ in Eq.~\ref{eq:private_model}. This parameter decides how much information back-fed from the proxy model $\overline{\mathbf{w}_i}$ to the private model $\mathbf{w}_i$. Recall that $\overleftarrow{\mathcal{KD}}_i$ demonstrates the selective knowledge from the high-certainty prediction of the proxy model. However, the high-certainty is only based on the prediction results solely from the proxy model itself. If we do not carefully design the weighted hyperparameter $\beta$, it might boost or even hurt the performance of the private model, because: (1) due to the compact size and naturally limited capability of the proxy model, though we have selected the high-certainty class set $\Omega$, it does not guarantee the classes in it are convincing prediction results compared with the ground truth or the output of the powerful private model; (2) the proxy model parameters are uploaded to the server for aggregation and distributed back to the clients. The aggregated proxy model parameters may not be a good fit for each local client's private data. Furthermore, in the federated learning paradigm, the model parameters of both the proxy model and private model are iteratively updated, which leads the performance on the private data $\mathcal{D}_i$ to change with respect to the communication round. Thus, it is an emergency to set an adaptive value with the consideration of the two model status.

We conduct a consensus-based approach to determine the value of $\beta$. Denoting the high-certainty set of the private model $\mathbf{w}_i$ and the proxy model $\overline{\mathbf{w}_i}$ as $\Omega$ and $\overline{\Omega}$ respectively, we use Jaccard Index to quantify the similarity of the two sets:
\begin{equation}
    \beta_{i} = |\Omega_i \cap \overline{\Omega_i}|/|\Omega_i \cup \overline{\Omega_i}|.
\end{equation}

After that, we alternatively minimize $\mathcal{L}_i$ and $\overline{\mathcal{L}_i}$ by bi-optimizing one and fixing the other one in the local training for client $i$.

\begin{table}[t]
\caption{Key Notations.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{cl}
\toprule
Symbol  & Definition and description \\
          \midrule
$\mathcal{D}_i$ & the data of client $i$ \\
$N$ & the number of clients\\
$B$ & the number of active/selected clients\\
$E$ & local training epoch\\
$\mathbf{w}_{i,e}^{t}$ & the large model of client $i$ at local training epoch $e$ at $t$\\
$\overline{\mathbf{w}_{i,e}^{t}}$ & the proxy model of client $i$ at local training epoch $e$ at $t$\\
$\Omega_{i,e,k}$& the set of large model for client $i$ at local epoch $e$ for data $k$\\
$\overline{\Omega_{i,e,k}}$& the set of small model for client $i$ at local epoch $e$ for data $k$\\


\bottomrule
\end{tabular}}
\label{tab:notation}
\end{table}

\begin{algorithm}[h]
\SetAlgoLined
\DontPrintSemicolon
\Input{ Local data $\mathcal{D}_1,\mathcal{D}_2,..,\mathcal{D}_N$, the number of active clients $B$, communication rounds $T$, the number of local training epochs $E$,}
{Randomly sample $B$ active clients and their model parameters are denoted as $\{\mathbf{w}_{1}^{t},\mathbf{w}_{2}^{t},\cdots, \mathbf{w}_{B}^{t}\}$;}\\
\For{\textup{each $t\in [1, \cdots, T]$}}{
\kwClient{}{

\For{each $\mathcal{D}_i^{k} \in [\mathcal{D}_i^{1}, \mathcal{D}_i^{2}, \cdots, \mathcal{D}_i^{K}]$}{

\Omega_{i,e,k}^{t} = \text{CF}(\mathbf{w}_{i,e}^{t}, x_i, \phi)

}
then we calculate the data weight by:
\For{each $\mathcal{D}_i^{k} \in [\mathcal{D}_i^{1}, \mathcal{D}_i^{2}, \cdots, \mathcal{D}_i^{K}]$}{
\theta_{i,e,k}^{t} =  

}





\For {\textup{each $i\in [1, \cdots, B]$}}{
\textup{Conduct \textit{layer-wise ecomposition} on $\mathbf{w}_{t}^{n} = [(\mathbf{L}_{t,1}^n, O^n_1), \cdots, (\mathbf{L}_{t,H}^b, O^n_E)]$;}
}
\textup{Conduct \textit{function-driven layer grouping} with Eq. (4) to obtain $\{\mathcal{G}_{t}^1,\mathcal{G}_{t}^2, \cdots, \mathcal{G}_t^{K}\}$;}\\
\textup{Conduct \textit{reassembly candidate generation} to obtain $\{\mathbf{c}_t^1, \cdots, \mathbf{c}_t^M\}$ following $\mathcal{R}_1,\mathcal{R}_2, \mathcal{R}_3$, and $\mathcal{R}_4$;}\\
\textup{Conduct \textit{layer stitching} on the generated candidates;}\\
\textup{Conduct \textit{similarity calculation} on pairs of models with Eq. (5);}\\
\textup{Distribute the personalized models back to the clients accordingly.}\\

}
\kwServer{}{
\For {\textup{each $n\in [1, \cdots, B]$}}{
\For{\textup{each local epoch $e$ from 1 to $E_c$}}{
Update $\mathbf{w}_t^n$ with Eq. (6);}
}}
Upload $B$ models $\{\mathbf{w}_{i}^{t}\}$ back to the server;}

\caption{\text{Algorithm Flow of \ours.}}
\label{alg:whole_process}
\end{algorithm}











% In this subsection, we introduce how to obtain the hyperparameter $\beta$ in Eq.~\ref{eq:private_model}. This parameter decides how much information back-fed from the proxy model $\overline{{\mathbf{w}_i}}$ to the private model ${\mathbf{w}_i}$. Recall that $\overleftarrow{\mathcal{KD}}_i$ demonstrates the selective knowledge from the high-certainty prediction of the proxy model. However, the high-certainty is only based on the prediction results solely from the proxy model itself. If we do not carefully design the weighted hyperparameter $\beta$, it might boost or even hurt the performance of the private model, because: (1) due to the compact size and naturally limited capability of the proxy model, though we have selected the high-certainty class set $\omega$, it does not guarantee the classes in it are convincing prediction results compared with the ground truth or the output of the powerful private model; (2) the proxy model parameters are uploaded to the server for aggregation and distributed back to the clients. The aggregated proxy model parameters may not be a good fit for each local client's private data. Furthermore, in the federated learning paradigm, the model parameters of both the proxy model and private model are iteratively updated, which leads the performance on the private data $\mathcal{D}_i$ to change with respect to the communication round. Thus, it is an emergency to set an adaptive value with the consideration of the two model status.











==> section/method_epoch.tex <==

\section{Methodology}
\subsection{Overview}
As illustrated in Figure~\ref{}(a), the proposed \ours framework comprises two key components: local update and server update. Local client $i$'s training data is denoted as $\overline{\mathcal{D}}_i$, we split the training data into 90\% for training the proxy model and the client model denoted as $\mathcal{D}_i$ and the 10\% for the conformal learning denoted as $\mathcal{D}^{c}_i$ in Section~\ref{sec:usp}. During each communication round $t$, we conduct $R$ local training epochs. Based on this, we initialize the proxy model as $\mathbf{p}_i^{t}$ and the client model as $\mathbf{w}_i^{t}$ using the data $\mathcal{D}_i$ from the $i$-th client. It is essential to note that in model-heterogeneous federated learning, the structures of client models $\{\mathbf{w}_1^{t}, \cdots, \mathbf{w}_N^{t}\}$ differ from one another, where $N$ represents the number of clients. Conversely, the structures of proxy models $\{\mathbf{p}_1^{t}, \cdots, \mathbf{p}_N^{t}\}$ are uniform. Furthermore, it is worth mentioning that the parameter size of $\mathbf{p}_i^{t}$ is typically much smaller than that of $\mathbf{w}_i^{t}$. 

Only the learned proxy models $\{\mathbf{p}_1^{t}, \cdots, \mathbf{p}_N^{t}\}$\footnote{In this cross-device setting, we will randomly select $B \ll N$ clients at each communication round.} are transmitted to the server for model aggregation during the server update, leading to a significant reduction in communication costs.
The resulting aggregated model $\mathbf{p}_g^t$ is then disseminated to each client in the subsequent communication round as the initialized proxy model, denoted as $\mathbf{p}_i^{t+1} = \mathbf{p}_g^t$ ($\forall i \in [1, \cdots, N]$). These two updates are executed iteratively until \ours converges. Next, we provide the details of each update.

\subsection{Local Update via Uncertainty-based Asymmetrical Reciprocity Learning}\label{sec:UARL}
The inherent challenge posed by model heterogeneity renders the direct aggregation of uploaded client models unfeasible. Despite various proposed approaches for heterogeneous model aggregation~\cite{lin2020ensemble, yu2022resource, huang2022learn, li2019fedmd,yi2023fedgh}, as discussed in Section~\ref{sec:intro}, they still exhibit several limitations. In contrast to existing work, we present a simple yet novel uncertainty-based asymmetrical reciprocity learning (\texttt{UARL}) approach to tackle the challenges posed by model heterogeneity. 
As shown in Figure~\ref{}(b), \texttt{UARL} is a bidirectional knowledge distillation (KD)-based model. 

The forward KD (FKD) follows the traditional ``teacher-student'' knowledge distillation approach. In FKD, a small proxy/student model $\mathbf{p}_i^{t,r}$ is distilled from the large, private client/teacher model $\mathbf{w}_i^{t,r}$ using the client data $\mathcal{D}_i$ for the $i$-th client during the $r$-th training epoch. The forward loss can be formulated as follows:
\begin{equation}
    \overrightarrow{\mathcal{J}}_i^{t,r} = \sum_{j=1}^{|\mathcal{D}^{b}_i|}\text{KL}(\mathbf{w}_i^{t,r}(\mathbf{x}^{r}_{j,b})|| \mathbf{p}_i^{t,r}(\mathbf{x}^{r}_{j,b})),
\end{equation}
where $|\mathcal{D}_i^{b}|$ denotes the number of $b$-th batch data at $i$-th client, $\text{KL}(\cdot, \cdot)$ is the Kullback–Leibler divergence, and $\mathbf{x}^{r}_{j,b}\in \mathcal{D}_i^{b}$ represents the input data from the $b$-th batch of training data at training epoch $r$.

The backward KD (BKD) poses a challenge, as the capability of the small proxy model $\mathbf{p}_i^{t,r}$ is typically weaker than that of the large client model $\mathbf{w}_i^{t,r}$. Directly applying traditional knowledge distillation may lead to a degradation in the power of client models. To overcome this asymmetrical reciprocity issue, we introduce a novel uncertainty-based behavior imitation learning method to transfer diverse knowledge from the proxy model $\mathbf{p}_i^{t,r}$ to the client model $\mathbf{w}_i^{t,r}$. Further details can be found in Section~\ref{sec:bkd_loss}.


% \textcolor{blue}{here}
Let $\overleftarrow{\mathcal{J}}_i^{t,r}$ denote the backward KD loss. 
We then use the following loss function to train the $i$-th client at the $r$-th training epoch at communication round $t$:
\begin{equation}\label{eq:client_training}
    \mathcal{J}_i^{t,r} = \sum_{j=1}^{|\mathcal{D}^{b}_i|}\text{CE}(\mathbf{w}_i^{t,r}(\mathbf{x}_{j,b}^{r}), \mathbf{y}_{j,b}^{r}) + \overrightarrow{\mathcal{J}}_i^{t,r} + \overleftarrow{\mathcal{J}}_i^{t,r},
\end{equation}
where $\mathbf{y}_{j,b}^{r}$ denotes the vectorized ground truth obtained from the real label set $\mathcal{Y}_{j,b}^{r}$ of $\mathbf{x}_{j,b}^{r}$. The algorithm flow can be found in Algorithm~\ref{alg:uarl}.


\begin{algorithm}[ht]
\small
\SetAlgoLined
\DontPrintSemicolon

\Input{Communication round $t$, client data $\mathcal{D}_i$ and $\mathcal{D}^{c}_i$, client model $\mathbf{w}_i^t$, client proxy model $\mathbf{p}_i^t$, local training epoch $R$, local training data batch number $B$, hyperparameters}

% \For{\textup{each communication round }$t = 1,2,\cdots$,T}{

    \For{epoch $r = 1, 2, \cdots, R$}{

     Obtain conformal model for local model: \\
     $\mathbf{w}^{t,r}_{i,c} \longleftarrow \{\mathcal{D}^{c}_i, \mathbf{w}_i^{t,r}\}$ \\
     Obtain conformal model for proxy model: \\
     $\mathbf{p}^{t,r}_{i,c} \longleftarrow \{\mathcal{D}^{c}_i, \mathbf{p}_i^{t,r}\}$

    % \kwClient{}{
    % \# \textit{Small client update}\\
        \For{$b \in [1, \cdots, B]$}{
        \If{$t>1$}{$\mathbf{w}_{i,t}^s = \mathbf{w}^g_{t-1}$;}
            {Calculate $\mathcal{R}^s_{i,t}$ via Eq.~\eqref{eq:small_pub_classification}/Eq.~\eqref{eq:small_pub_segmentation} using the public data $\mathcal{D}_p$;\\
            Calculate $\mathcal{L}^s_{i,t} $ via Eq.~\eqref{eq:small_private_loss}/Eq.~\eqref{eq:small_seg_loss} using private data $\mathcal{D}_{i}$;\\
            \textup{Jointly optimize $\mathcal{R}^s_{i,t}$ and $\mathcal{L}^s_{i,t} $ by minimizing $\mathcal{J}_{i,t}^s$ via Eq~\eqref{eq:small_loss};
            }
        }

        }
        % \# \textit{Large client update}\\
        \For{$j \in [1, \cdots, N_l]$}{
        \If{$t>1$}{$\hat{\mathbf{w}}_{j,t}^l = \mathbf{w}^g_{t-1}$;}
            Calculate $\overrightarrow{\mathcal{KD}}_{j,t}^l$ via Eq.~\eqref{eq:large_forward}/Eq.~\eqref{eq:seg_forward};\\
            Calculate $\overleftarrow{\mathcal{KD}}_{j,t}^l$ via Eq.~\eqref{eq:ranking_KD}/Eq.~\eqref{eq:seg_backward};\\
            Update $\mathbf{w}^{l}_{j,t}$ by minimizing $\mathcal{G}_{j,t}^l$ via Eq.~\eqref{eq:large_loss};
        }

        
        Upload $\{\mathbf{w}_{1,t}^s, \cdots, \mathbf{w}_{N_s,t}^s\}$ and $\{\hat{\mathbf{w}}_{1,t}^l, \cdots, \hat{\mathbf{w}}_{N_l,t}^l\}$ to the server;
    
% }

    % \kwServer{}{
    %     \textup{Obtain the aggregated model $\mathbf{w}^g_t$ via FedAvg;}\\
    %     \textup{Distribute the aggregated model $\mathbf{w}^g_t$ back to clients.}
    % }
    }

\caption{Algorithm Flow of \texttt{UARL}. \textcolor{blue}{ to be updated}}
\label{alg:uarl}
\end{algorithm}



\subsection{Uncertainty-based Behavior Imitation Learning}\label{sec:bkd_loss}
The initialization of the proxy model $\mathbf{p}_i^{t}$ is carried out using the aggregated global model $\mathbf{p}_g^{t-1}$ (refer to Section~\ref{sec:server_update})\footnote{To help the demonstration more clear, we use $\mathbf{p}_i^{t}$ to generally define the proxy model we have at communication round $t$. When we describe the specific training process, we add the epoch information into the notation, e.g., $\mathbf{p}_i^{t,r}$ for the $r$-th training epoch. The same as $\mathbf{w}_i^t$ and $\mathbf{w}_i^{t,r}$,  $\mathcal{S}_j^t$ and  $\mathcal{S}_j^{t,r}$.}. This global model encapsulates diverse knowledge from other clients, making it crucial to transfer this knowledge to the private client model. However, due to the inherently weaker capability of the proxy model $\mathbf{p}_i^t$, direct application of the traditional ``teacher-student'' learning paradigm for knowledge transfer to the large model $\mathbf{w}_i^t$ is impractical. Such a direct approach may introduce additional noise to the large model, potentially impeding the overall training efficiency of the entire framework.

\subsubsection{Backward Knowledge Distillation Loss}
To tackle this challenge, we introduce an uncertainty-based behavior imitation learning approach at each local training epoch. This method exclusively relies on the use of \textbf{partial logits} generated by the proxy model $\mathbf{p}_i^{t,r}$ with a high level of confidence or certainty. The intention is to employ these confident predictions to guide the learning process of the large model $\mathbf{w}_i^{t,r}$ at each local training epoch $r$.
In essence, given a batch of training data $\mathcal{D}_i^{b} \in \mathcal{D}_i$, when dealing with a specific of data $\mathbf{x}_{j,b}^{r} \in \mathcal{D}_i^{b}$, if the proxy model $\mathbf{p}_i^{t,r}$ exhibits high confidence in predicting certain classes, transferring this behavioral information—rather than the complete logits—can still be beneficial for the training of the large model.

Let $\mathcal{S}_{j,b}^{t,r}$ represent the set of class labels predicted with high confidence by $\mathbf{p}_i^{t,r}$ on data $\mathbf{x}_{j,b}^{r}$ from the $b$-th batch at the $r$-th training epoch. In our proposed behavior imitation learning, the objective is to strengthen the probability/logit associated with the labels in $\mathcal{S}_{j,b}^{t,r}$ as predicted by the large model $\mathbf{w}_i^{t,r}$. Importantly, we refrain from imposing a strict requirement for the large model $\mathbf{w}_i^{t,r}$ to prioritize ranking the labels in $\mathcal{S}_{j,b}^{t,r}$ at the top positions. To address this, we introduce a novel ranking-based behavior imitation learning loss, outlined as follows:
\begin{equation}\label{eq:certainty_KD}
\small
\begin{split}
    &\overleftarrow{\mathcal{J}}_i^{t,r} = \sum_{j=1}^{|\mathcal{D}^{b}_i|} \eta_{j,b}^{t,r} \sum_{k \in \mathcal{S}_{j,b}^{t,r}} \log(\frac{\exp(\mathbf{w}_i^{t,r}(\mathbf{x}^{r}_{j,b})[k])}{\Phi_j^{t,r}}),\\
    \Phi_j^{t,r} = &\sum_{s \in \mathcal{S}_{j,b}^{t,r}} \exp(\mathbf{w}_i^{t,r}(\mathbf{x}^{r}_{j,b})[s]) + \sum_{v \in \mathcal{V}_{j,b}^{t,r}} \exp(\mathbf{w}_i^{t,r}(\mathbf{x}^{r}_{j,b})[v]),
\end{split}
\end{equation}
where $\mathbf{w}_i^{t,r}(\mathbf{x}^{r}_{j,b})[k]$ denotes the logit value of the $k$-th label in the prediction.
$\eta_{j,b}^{t,r}$ is the estimated consensus weight to determine the amount of the transferred knowledge from the proxy model $\mathbf{p}_i^{t,r}$ to the large model $\mathbf{w}_i^{t,r}$.
$\mathcal{V}_j^{t,r} = \mathcal{Y} - \mathcal{S}_j^{t,r}$ denotes the class labels associated with low confidence, and $\mathcal{Y}$ represents the complete set of class labels in $\mathcal{D}^{b}_i$. 
In Eq.~\eqref{eq:certainty_KD}, $\eta_{j,b}^{t,r}$ and $\mathcal{S}_j^{t,r}$ are unknown variables. 
To proceed, we introduce a novel approach to quantify an uncertainty set $\mathcal{S}_j^{t,r}$ for each data $\mathbf{x}^{r}_{j,b}$ through dynamic conformal prediction, and the uncertainty sets will be further used to estimate $\eta_{j,b}^{t,r}$.

% \textcolor{blue}{here}

\subsubsection{Uncertainty Set Prediction}\label{sec:usp}
Conformal prediction~\cite{angelopoulos2020uncertainty} stands out as a reliable and interpretable approach for quantifying uncertainty, providing prediction sets accompanied by a designated level of confidence or probability. In mathematical terms, conformal prediction involves an uncertainty set function $f(\mathbf{p}_j^t, \mathbf{x}_j)$ that maps $\mathbf{x}_j$ to a subset of $\mathcal{Y}$ (i.e., $f(\mathbf{p}_j^{t}, \mathbf{x}_j) = \mathcal{S}_j^t \in \mathcal{Y}$), satisfying the condition:
\begin{equation}
    P(\mathcal{Y}_j \in \mathcal{S}_j^t)) \geq 1-\theta,
\end{equation}
where $\theta$ represents a predefined confidence level. 

All existing conformal prediction approaches are designed to quantify uncertainty for well-trained models on unseen samples~\cite{}. In order words, these classifiers remain fixed. However, the \ours framework undergoes iterative training, resulting in dynamic changes to the models $\mathbf{p}_i^t$ and $\mathbf{w}_i^t$ at each communication round.\footnote{In our implementation, the parameters of two models change at each epoch $r$ during each communication round $t$ in the training stage. Here, we omit the notation of epoch $r$ in the rest of this section for simplicity and readability, which can be treated as $r=1$ in each communication round $t$.} Consequently, the uncertainty set $\mathcal{S}_j^{t}$ is predicted dynamically.

A straightforward approach would involve directly applying existing conformal prediction methods, such as regularized adaptive prediction sets (RAPS)~\cite{angelopoulos2020uncertainty}, to generate the uncertainty set $\mathcal{S}_{j,b}^{t,r}$ for $\mathbf{x}^{r}_{j,b}$ at local training epoch $r$ of communication round $t$. However, as mentioned earlier, the capability of the proxy model $\mathbf{p}_i^{t,r}$ is weak, especially at the initial stages of training. Utilizing prediction sets from such unreliable models may introduce adverse effects when training Eq.~\eqref{eq:certainty_KD}.

To address this challenge, we introduce a dynamic adjustment mechanism for the size of the prediction set $\mathcal{S}_{j}^{t,r}$ based on the observed changes in model performance on the training data $\mathbf{x}^{r}_{j,b}$ from $\mathcal{D}^{b}_i$. In essence, a decrease in a model's performance may be indicative of incorrect or low-quality prediction sets. Therefore, the size of the prediction sets needs to be reduced, ensuring guarantees on the predicted labels with high confidence.
Based on this intuition, we propose a dynamic conformal prediction for federated learning training based on RAPS using the following uncertainty prediction set generation:
\begin{equation}\label{eq:cp}
    \begin{split}
        \mathcal{S}_{j.b}^{t,r} &:= 
        \{y : \pi_j(y) \cdot u + \rho_j(y) \\
        &+ g(\Delta^{t,r}, \lambda_{b}^{t,r}) \cdot (o_j(y)-k_{reg})^{+} \leq \tau\}.
    \end{split}
\end{equation}
$\pi_j(y)$ represents the probability assigned to the label $y$ as predicted by the model $\mathbf{p}_i^{t,r}$ for the $j$-th data point $\mathbf{x}^{r}_{j,b}$. The parameter $u$ is a predefined randomized factor determining the value jump for each new label $y$.
Furthermore, $\rho_j(y) = \sum_{y^\prime=1}^{|\mathcal{Y}|} \pi_j(y^\prime) \mathbbm{1}_{\{\pi_j(y^\prime) > \pi_j(y)\}}$ denotes the total probability mass associated with the set of labels that are more likely than the label $y$.

Besides, $g(\Delta^{t,r},  \lambda^{t,r})$ is a piecewise calibration function\footnote{Here, we define a simple linear function to characterize the dynamic adjustment of prediction set. We can also use other monotonically decreasing functions as alternative solutions.}, which is defined as follows:
\begin{equation}
    g(\Delta^{t,r},\lambda^{t,r}) = 
    \begin{cases}
        \lambda^{t,r} \cdot \Delta^{t,r} - \Delta^{t,r} + \lambda^{t,r}, &\text{if $\Delta^{t,r} < 0$,}\\
        \lambda^{t,r}, &\text{otherwise}.
    \end{cases}
\end{equation}
$\Delta^{t,r} = \mathcal{A}(\mathbf{p}_i^{t,r}, \mathcal{D}^{b}_i) - \mathcal{A}(\mathbf{p}_i^{t-1}, \mathcal{D}^{b}_i)$, where $\mathcal{A}(\mathbf{p}_i^{t}, \mathcal{D}^{b}_i)$ denotes the training accuracy on $\mathcal{D}^{b}_i$ using the trained model $\mathbf{p}_i^{t,r}$. 
In the event of a performance drop, i.e., $\Delta^{t,r} < 0$, we actively reduce the size of the prediction set by adjusting the value of $g(\Delta^{t,r}, \lambda^{t,r})$. On the other hand, if $\Delta^{t,r} \geq 0$, we maintain $g(\Delta^{t,r}, \lambda^{t,r}) = \lambda^{t,r}$, where $\lambda^{t,r} \geq 0$ serves as a predefined regularization hyperparameter.

In addition, $(z)^+$ denotes the positive part of $z$, and $k_{reg}$ is another regularization hyperparameter. The variable $o_j(y)=|y^\prime \in \mathcal{Y}: \pi_j(y^\prime) \geq \pi_j(y)|$ represents the ranking of $y$ among the labels in $\mathcal{Y}$ based on the prediction probability $\pi_j$. Finally, $\tau$ denotes the cumulative sum of the sorted, penalized classifier scores. The details of the designed dynamic conformal prediction can be found in Appendix~\ref{XXX}.

% \textcolor{blue}{here}

\subsubsection{Consensus Weight Estimition}\label{sec:weight}
In Eq.~\eqref{eq:certainty_KD}, $\eta_j^{t,r}$ is a key factor to control the behavior of knowledge transfer from the proxy model $\mathbf{p}_i^{t,r}$ to the large model $\mathbf{w}_i^{t,r}$. Intuitively, if the proxy model $\mathbf{p}_i^{t,r}$ is significantly confident on certain predicted labels on data $\mathbf{x}^{r}_{j,b}$ i.e., the small size of $\mathcal{S}_{j,b}^{t,b}$, then it is necessary to transfer such high-quality knowledge to the large model $\mathbf{w}_i^{t,r}$ as much as possible, as the guidance of model training. On the other hand, we need to reduce the amount of transferred knowledge with low quality, i.e., the uncertainty set $\mathcal{S}_{j,b}^{t,b}$ with large size. 

The quality of knowledge is a relative variable, which can be determined by the size of uncertainty sets predicted by both models $\mathbf{p}_i^{t,r}$ and $\mathbf{w}_i^{t,r}$ on $\mathcal{S}_{j,b}^{t,b}$ using Eq.~\eqref{eq:cp}, denoted as $\mathcal{S}_{j,b}^{t,r}$ and $\mathcal{L}_{j,b}^{t,r}$, respectively. Mathematically, we define the consensus weight $\eta_j^{t,r}$ as follows:
\begin{equation}\label{eq:eta}
    \eta_{j,b}^{t,r} = 
    \begin{cases}
        |\mathcal{S}_{j,b}^{t,r} \cap \mathcal{L}_{j,b}^{t,r}/|\mathcal{S}_{j,b}^{t,r} \cup \mathcal{L}_{j,b}^{t,r}|, & \text{if $|\mathcal{S}_{j,b}^{t,r}| \geq |\mathcal{L}_{j,b}^{t,r}|$},\\
       |\mathcal{S}_{j,b}^{t,r} \cap \mathcal{L}_{j,b}^{t,r}|/|\mathcal{L}_{j,b}^{t,r}|, & \text{if $|\mathcal{S}_{j,b}^{t,r}|<|\mathcal{L}_{j,b}^{t,r}|$},
    \end{cases}
\end{equation}
where $|\cdot|$ denotes the size of the set. We can observe that such a design encourages the proxy model to transfer confident knowledge to the large model.

\subsection{Server Update}\label{sec:server_update}
After training each client using Eq.~\eqref{eq:client_training}, we will obtain both proxy and private models. The proxy models $\{\mathbf{p}_1^t, \cdots, \mathbf{p}_N^t\}$ will be uploaded to the server to conduct aggregation, resulting in a share proxy global model $\mathbf{p}_g^t$ using any existing data-free aggregation approaches, such as FedAvg~\cite{mcmahan2017communication} and FedProx~\cite{li2020federated}. The global model $\mathbf{p}_g^t$ will be distributed to each client at the next communication round as the initialization of the proxy client model, i.e., $\mathbf{p}_i^{t+1} = \mathbf{p}_g^t$. The proposed \ours framework will be iteratively executed for the client update and server update until convergence. 


==> section/others.tex <==
\*section{Broader Impact}

==> section/rebuttal.tex <==
\newpage

\onecolumn

\section*{Reviewer i7Zn}
Thanks for the reviewer's constructive comments. We will address the concerns one by one as follows.
\subsection*{W1}

In our review of related work, we noted that FedRolex imposes a limitation requiring client models to be subsets of a global model. HeteroFL shares this same limitation. Our methodology, however, is not bound by such constraints, affording greater flexibility in the selection of client models, which may not fall into the same specific research track as the sub-model track.


As for the second point of the performance change with respect to the model size, we have conducted the study of different sizes and types of proxy models in Sec 4.2.5 and Table 3. We observe that the performance is generally boosted with the increase of the proxy model size. To further address the reviewer's question, we utilize the largest model VGG-19 from the model pool as the client's private model and maintain all the other settings as Table 1. We report the results on CIFAR-10 dataset ($\alpha = 0.5$) as follows. In some cases, the performance of the proxy model and global model will has a little bit drop. The reason might be that the knowledge distillation will be affected by the model structures of the teacher model and student model. As the proxy model is ResNet 18, our original experiment results, 
 which are based on the private model pool containing ResNet and VGG, would show a superior performance of the proxy models and global models.  However, We observe that the performance of the private model gets boosted in most cases, due to the model capability and complexity of VGG-19 as the private model with the local training. 




\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{Private models are all VGG-19 in our framework. FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\toprule 
&  \multicolumn{3}{c|}{\textbf{FedAvg}}&
\multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ 
   & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
      \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
      Our + VGG &-&-&92.86&-&-&94.05&-&-&94.26&-&-&94.87\\
      Our + VGG19& 83.98&89.67&91.35&86.20&
94.16&94.12&86.77&91.84&93.45&87.19&91.24&
94.33\\
      Our &83.93&89.45&91.22&86.44&91.50
&93.84&87.13&92.05&92.36&87.85&92.11
&93.17
\\\hline
   \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
\midrule
Our + VGG &-&-&87.89&-&-&88.62&-&-&89.10&-&-&89.92\\
Our + VGG19& 63.04&82.33&87.04&66.16&
82.69&87.80&65.77&83.11&87.98&66.21&84.13&89.55
\\
Our&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
83.00&87.24&66.87&84.49&88.67\\\hline
   \multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
   Our + VGG &-&-&65.91&-&-&67.52&-&-&69.81&-&-&69.98\\
   Our + VGG19& 38.87&61.29&65.77&39.86&61.00&66.71&41.89&62.73&67.89&42.03&63.58&68.89\\
   Our &38.17&
61.06&65.69&39.31&61.22&65.45&40.92&62.68&
67.07&41.24&62.96&67.35\\\hline
   \multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
   Our + VGG &-&-&56.89&-&-&58.94&-&-&59.06&-&-&59.22\\
   Our + VGG19& 43.21&53.26&56.62&43.56&53.89&57.12&42.98&
54.10&57.59&42.74&54.85&57.96\\
Our&42.30&	53.48&	55.95&
41.77&	54.30&	56.86&
42.35&	53.85&	56.68&
41.82&	54.04&	57.21\\
\bottomrule 
\end{tabular}
}
\label{tab:app_largest}
\vspace{-0.1in}
\end{table*}


% We also provide another type of upper bound of the system. 



% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{Homo private models are all VGG-19. We conduct the basic FL.FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c} 
% \toprule 
% &  \multicolumn{1}{c|}{\textbf{FedAvg}}&
% \multicolumn{1}{c|}{\textbf{FedProx}} & \multicolumn{1}{c|}{\textbf{pFedMe}} & \multicolumn{1}{c}{\textbf{pFedBayes}}\\ \hline

%       \multicolumn{5}{c}{\textbf{FMNIST}} \\\hline
%       Homo VGG19 &92.86&94.05&94.26&94.87\\
%       Our &91.22
% &93.84&92.36&93.17
% \\\hline
%    \multicolumn{5}{c}{\textbf{CIFAR-10}} \\
% \midrule
% Homo VGG19&
% \\
% Our&86.83&86.92&87.24&88.67\\\hline
%    \multicolumn{5}{c}{\textbf{CIFAR-100}} \\\hline
%    Homo VGG19&65.91&67.52&69.81&69.98\\
%    Our &65.69&65.45&67.07&67.35\\\hline
%    \multicolumn{5}{c}{\textbf{FedISIC-19}} \\\hline
%    Homo VGG19&56.89&58.94&59.06&59.22\\
% Our&55.95&
% 56.86&
% 56.68&
% 57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_largest_homo}
% \vspace{-0.1in}
% \end{table*}


















\subsection*{W2}

We agree that a key rationale behind adopting heterogeneous models in FL is the variation in clients' model training capabilities. However, model heterogeneity is also prevalent in real-world applications, including those cross-silo settings where clients' capability variances are minimal. Additionally, the paper highlights several advantages of employing proxy models: (1) Proxy models prevent the full disclosure of the structure and parameters of private models, thereby bolstering privacy. (2) Typically, proxy models are smaller than the private models maintained locally. This size difference means that transmitting proxy models between the server and clients can significantly reduce communication overhead in the FL framework.

\subsection*{W3}

Due to space constraints, our empirical convergence analysis is detailed in Appendix G and illustrated in Figure 5. In future research, we intend to delve into the theoretical convergence analysis of the entire framework.








\subsection*{Q1}
Thanks for the question, we have addressed it in the response to the weakness 1 as above.

\subsection*{Q2}
Thanks for the question, we have addressed it in the response to the weakness 2 as above.


\section*{Reviewer JJT3}

\subsection*{W1}

We carried out experiments on the CIFAR-10 dataset with $\alpha = 0.5$, employing an increasing function g() in the range [0,1], defined as$g = 0.5 \cdot \Delta^t + 0.5$, while keeping all other settings consistent with those described in Figure 3. The outcomes are reported in the subsequent table:

\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{New g() function. CIFAR-10 dataset with $\alpha = 0.5$}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\toprule 
&  \multicolumn{3}{c|}{\textbf{FedAvg}}&
\multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ \hline

   & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
    \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
    New g()&82.65&89.11&91.00&85.27&91.13&92.92
&86.06&91.58&92.25&86.45&91.89&93.08\\
    Our &83.93&89.45&91.22&86.44&91.50
&93.84&87.13&92.05&92.36&87.85&92.11
&93.17\\\hline
   \multicolumn{13}{c}{\textbf{CIFAR-10}} \\\hline
   
   

New g()&61.04&80.26&83.11&63.43&81.79&84.60&
64.51&82.36&86.47&66.52&83.61&86.80\\
Our g()&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
83.00&87.24&66.87&84.49&88.67\\\hline
\multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
    New g()&35.5&58.31&62.45&37.88&58.93&63.22&37.69&60.14&66.85&41.11&61.64&66.57\\
    Our g()&38.17&
61.06&65.69&39.31&61.22&65.45&40.92&62.68&
67.07&41.24&62.96&67.35\\\hline
\multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
New g()&36.7&44.14&50.62&36.81&46.65&53.52&
38.03&48.25&53.48&37.66&47.89&53.17\\
Our g()&42.30&	53.48&	55.95&
41.77&	54.30&	56.86&
42.35&	53.85&	56.68&
41.82&	54.04&	57.21\\
\bottomrule 
\end{tabular}
}
\label{tab:app_new_g}
\vspace{-0.1in}
\end{table*}




We observe that the performance will be harmed if the g() function is an increasing one. This further demonstrates the reasonable design of the calibration function.

\subsection*{W2}
Thanks for pointing it out. The results are calculated on the testing set. We will add specific descriptions in the updated version of the paper to avoid confusion.

\subsection*{W3}



Thank you for posing this insightful question. We've illustrated the empirical convergence through Figure 5, which shows the progression of the value of $\eta$ across different communication rounds. By examining the interplay between the data in Figures 5 and 6, it is evident that $\eta$ increases as the system gradually approaches convergence through successive communication rounds. Moreover, once the system nears convergence, the value of $\eta$ stabilizes close to, or exactly at, 1. Given $\eta$'s role in quantifying the consensus level between the proxy and private models, its correlation with system convergence underscores the effectiveness and logical foundation of our approach. This alignment affirms the integrity of our design's impact on achieving consensus and system convergence.

\subsection*{W4}

Due to constraints on page length, our discourse on resource consumption is located in Appendix M. Here, we assess computational efficiency by measuring training duration. Although our method slightly extends training time compared to the traditional symmetrical KD loss, this minor increase is counterbalanced by a noticeable enhancement in performance, as evidenced in the ablation study detailed in Section 4.2.3.


\section*{Reviewer ytUi}


\subsection*{W1}
As highlighted by the reviewer, we discussed the landscape of heterogeneous federated learning in Section 2.1. The techniques outlined in the second paragraph necessitate the exchange of additional data, like class scores and label-wise representations, potentially elevating privacy risks. In contrast, our method requires only the sharing of proxy model parameters, steering clear of transmitting any client-sensitive information. Nevertheless, we would like to evaluate and contrast these methods in future studies, to ascertain their importance in achieving optimal performance, as recommended by the reviewer.

As the reviewer suggested, we conducted the experiment of the baseline FedMD and FCCL. Both of them need to exchange extra information between the server and the clients and use public data. FedMD uses the labeled public data and FCCL uses the unlabeled public data. Following the setting in the paper FedMD, we use the CIFAR-10 as the public dataset and the CIFAR-100 as the private dataset. With maintaining all the other settings the same as our main paper, we report the results as follows




% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{FedMD. FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc} 
% \toprule 
% &  \multicolumn{3}{c|}{\textbf{FedAvg}}&
% \multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ 
%    & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
%       \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
%       Our + VGG &-&-&92.86&-&-&94.05&-&-&94.26&-&-&94.87\\
%       Our + VGG19& 83.98&89.67&91.35&86.20&
% 94.16&94.12&86.77&91.84&93.45&87.19&91.24&
% 94.33\\
%       Our &83.93&89.45&91.22&86.44&91.50
% &93.84&87.13&92.05&92.36&87.85&92.11
% &93.17
% \\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
% \midrule
% Our + VGG &-&-&87.89&-&-&88.62&-&-&89.10&-&-&89.92\\
% Our + VGG19& 63.04&82.33&87.04&66.16&
% 82.69&87.80&65.77&83.11&87.98&66.21&84.13&89.55
% \\
% Our&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
% 83.00&87.24&66.87&84.49&88.67\\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
%    Our + VGG &-&-&65.91&-&-&67.52&-&-&69.81&-&-&69.98\\
%    Our + VGG19& 38.87&61.29&65.77&39.86&61.00&66.71&41.89&62.73&67.89&42.03&63.58&68.89\\
%    Our &38.17&
% 61.06&65.69&39.31&61.22&65.45&40.92&62.68&
% 67.07&41.24&62.96&67.35\\\hline
%    \multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
%    Our + VGG &-&-&56.89&-&-&58.94&-&-&59.06&-&-&59.22\\
%    Our + VGG19& 43.21&53.26&56.62&43.56&53.89&57.12&42.98&
% 54.10&57.59&42.74&54.85&57.96\\
% Our&42.30&	53.48&	55.95&
% 41.77&	54.30&	56.86&
% 42.35&	53.85&	56.68&
% 41.82&	54.04&	57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_baseline}
% \vspace{-0.1in}
% \end{table*}

\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{Baselines on CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}
{
\begin{tabular}{c|c|c|c|c|c|c} 
\toprule 
Approach & Public Data &Extra Information&{\textbf{FedAvg}}&
{\textbf{FedProx}} & {\textbf{pFedMe}} & {\textbf{pFedBayes}}\\ \hline



FedType&No& No &65.69&65.45&67.07&67.35\\\hline
FedMD&Yes&Yes& \multicolumn{4}{c}{65.82}\\



\bottomrule 
\end{tabular}
}
\label{tab:app_baseline}
\vspace{-0.1in}
\end{table*}




\subsection*{W2}
Thanks for the reviewer's constructive suggestion. In our existing experiment results, we use ResNet-18 as the proxy model and the local private models cover ResNet-18, ResNet-34,
ResNet-50, RestNet-101, ResNet 152, VGG-11, VGG-13,
VGG-16, and VGG-19. To address the reviewer's question, we conduct the experiments ($\alpha = 0.5$, the proxy model is ResNet-18) with maintaining all the same settings as Table 1 except (1) FedType (ResNet): we only keep the ResNet family models in the model pool including ResNet-18, ResNet-34,
ResNet-50, RestNet-101, and ResNet 152; (2) FedType (VGG) we only keep the VGG family models in the model pool including VGG-11, VGG-13, VGG-16, and VGG-19. We report the results in the following table.



\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{All the clients' personal models are from ResNet family models or the VGG family models.  FMNIST/CIFAR-10/CIFAR-100 with $\alpha = 0.5$/Fed-ISIC dataset}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\toprule 
&  \multicolumn{3}{c|}{\textbf{FedAvg}}&
\multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\\hline 
   & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
    \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
    FedType(VGG)&83.22&88.87&90.86&84.31&91.07&92.46
&86.65&91.77&92.20&87.04&91.98&92.46\\
    FedType (ResNet)&84.55&89.63&91.12&85.51&91.86&93.61&87.41
&93.55&93.64&87.62&92.33&94.86\\
    FedType  &83.93&89.45&91.22&86.44&91.50
&93.84&87.13&92.05&92.36&87.85&92.11
&93.17\\\hline
   \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
\hline
FedType(VGG)&61.22&80.61&83.07&64.95&80.87&84.14
&63.40&81.36&84.52&65.48&81.27&86.11\\
FedType (ResNet)&64.59&83.62&86.88&66.11&83.79&87.25&66.89&84.08&87.10&67.03&
84.55&88.96\\
FedType&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
83.00&87.24&66.87&84.49&88.67\\\hline
\multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
FedType(VGG)&35.96&58.74&62.41&36.77&58.91&62.88
&39.52&59.61&63.05&40.08&61.63&63.85\\
    FedType (ResNet)&38.95&62.48&65.53&40.66&63.07&
67.89&41.56&62.97&68.16&41.82&63.57&67.94\\
    FedType&38.17&
61.06&65.69&39.31&61.22&65.45&40.92&62.68&
67.07&41.24&62.96&67.35\\\hline
\multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
FedType(VGG)&40.76&51.06&52.90&42.04&51.98&53.69
&42.13&52.61&53.12&41.01&52.48&54.55\\
FedType(ResNet)&42.86&53.55&55.84&42.84&
55.51&56.90&42.21&53.88&57.03&42.37&55.22&
57.10\\
FedType&42.30&	53.48&	55.95&
41.77&	54.30&	56.86&
42.35&	53.85&	56.68&
41.82&	54.04&	57.21\\
\bottomrule 
\end{tabular}
}
\label{tab:app_resnet}
\vspace{-0.1in}
\end{table*}


Based on the findings, it is evident that performance metrics, when using ResNet or VGG model families, tend to be superior or inferior compared to our initially reported outcomes. This observation corroborates the reviewer's insights regarding performance enhancements or declines resulting from the model's architectural congruence with KD techniques. These outcomes further validate the robustness and adaptability of our proposed framework across diverse conditions.



% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{All the clients' personal models are from VGG family models.  FMNIST/CIFAR-10/CIFAR-100 with $\alpha = 0.5$/Fed-ISIC dataset}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc} 
% \toprule 
% &  \multicolumn{3}{c|}{\textbf{FedAvg}}&
% \multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ 
%    & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
%     \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
%     FedType (VGG)&84.55&89.63&91.12&85.51&91.86&93.61&87.41
% &93.55&93.64&87.62&92.33&94.86\\
%     FedType  &83.93&89.45&91.22&86.44&91.50
% &93.84&87.13&92.05&92.36&87.85&92.11
% &93.17\\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
% \hline
% FedType (VGG)&64.59&83.62&86.88&66.11&83.79&87.25&66.89&84.08&87.10&67.03&
% 84.55&88.96\\
% FedType&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
% 83.00&87.24&66.87&84.49&88.67\\\hline
% \multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
%     FedType (VGG)\\
%     FedType&38.17&
% 61.06&65.69&39.31&61.22&65.45&40.92&62.68&
% 67.07&41.24&62.96&67.35\\\hline
% \multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
% FedType(VGG)&42.86&53.55&55.84&42.84&
% 55.51&56.90&42.21&53.88&57.03&42.37&55.22&
% 57.10\\
% FedType&42.30&	53.48&	55.95&
% 41.77&	54.30&	56.86&
% 42.35&	53.85&	56.68&
% 41.82&	54.04&	57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_vgg}
% \vspace{-0.1in}
% \end{table*}














\subsection*{Q}
We apologize for the typos. You are correct. Figure 4.3 should be Figure and FedERAL should be FedType. We will fix the typos in the updated version of the paper.


\section*{Reviewer i2GH}

\subsection*{Q1}
We totally agree with the reviewer that the basic mutual learning in FL has been developed. In our designed approach, we designed a novel uncertainty-based asymmetrical reciprocity learning to conduct the bi-directional learning, which considers the model size and the information diversity they carry. In our ablation study (Sec 4.2.3), FedType\_sym can be treated as a traditional mutual learning setting and our approach shows superior performance over it on the CIFAR-10 and Fed-ISIC 19 datasets in Table 2. 






\subsection*{Q2}
Thanks for pointing out. We will add them to our related work section in our updated version paper.

\subsection*{Q3}
We express our gratitude for the insightful feedback provided by the reviewer. The referenced baseline, FML, has been evaluated alongside our methodology in the ablation study within the context of FedType\_sym, where we implement a conventional knowledge distillation process. We intend to incorporate additional notes in the updated version of our paper to clarify this comparison further.

\subsection*{Q4}

Thanks for the reviewer's suggestion. We provide the communication cost reduction results shown in Sec 4.3 and Figure 4. Compared with exchanging the clients' private model parameters, our approach only transmits around 8\% of baselines' parameters with maintaining comparable performance. As for the computational cost, due to the page limit, we provide the quantitative results in Appendix M using the training time compared with different training losses. The results demonstrate that our approach is able to boost the performance with a limited extra computational time.  In line with the reviewer's advice, we aim to further decrease the computational cost in our subsequent research efforts.






==> section/rebuttal_new.tex <==
\newpage

\onecolumn


\textcolor{blue}{NEW!!!!!!!!!!!}
\section*{Reviewer i7Zn}
Thanks for the reviewer's constructive comments. We will address the concerns one by one as follows.
\subsection*{W1 \& Q1}

$\bullet$ \textbf{Baselines}. Thanks for pointing out the two representative approaches: FedRolex and HeteroFL. These two studies aim to collaboratively train a large, shared global model by distributing submodels to clients, where the heterogeneous submodels are part of the large global model. Besides, during the model learning, the structures of the distributed submodels to clients will change in different communication rounds, but the shared global model is fixed.

However, our setting is significantly different from theirs as follows:
(1) \textbf{The learning objective is different}. Our goal is to boost the performance of each local client with the federated learning paradigm instead of learning a shared global model. Thus, our work can be treated as the problem of personalized model heterogeneity in federated learning.
(2) \textbf{The way of model deployment is different}. In our setting, we fix the model structures of clients during the learning but allow clients to hold different types of models, such as ResNet and VGG, used in the experiments. The learning direction of our setting is from bottom to up. 
On the contrary, existing work requires a fixed global model, which distributes a random submodel to each client in each communication round. In other words, the client may use different models throughout the learning, but they are all subsets of the same global model. These approaches can be considered as the top-down learning paradigm.

Therefore, although training FedRolex and HeteroFL does not need public data, our experimental setting, where clients hold different types of models, still makes them unworkable. Thus, we did not compare them in the experiments.

$\bullet$ \textbf{Upper bound performance}. The upper-bound performance will be obtained by training the federated learning framework in the homogeneous setting, where each client uses the largest model (i.e., VGG-19 in our experiments). Since the homogeneous setting aims to train a shared global model, we report the average performance tested on each client with the learned global model from \textbf{Homo-VGG-19} in the following table, compared with the performance of private models obtained by our proposed FedType with $\alpha = 0.5$. To maximize the performance of the private model with our setting, we also tested another model, named \textbf{VGG-19+ResNet-18}, in which all clients used VGG-19 as the private model and ResNet-18 as the proxy model. 

\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{Private models are all VGG-19 in our framework. FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}
{
\begin{tabular}{c|c|c|c|c|c} 
\toprule 
Dataset & Model & {\textbf{FedAvg}}&
{\textbf{FedProx}} & {\textbf{pFedMe}} & {\textbf{pFedBayes}}\\ \hline

\multirow{3}{*}{\textbf{FMNIST}} 
& Homo-VGG-19 &92.86&94.05&94.26&94.87\\
%       Our + VGG19& 83.98&89.67&91.35&86.20&
% 94.16&94.12&86.77&91.84&93.45&87.19&91.24&
% 94.33\\
& VGG-19+ResNet-18 & 91.35& 94.12&93.45&94.33\\
&FedType &91.22&93.84&92.36&93.17
\\\hline

\multirow{3}{*}{\textbf{CIFAR-10}} 
& Homo-VGG-19 & 87.89&88.62&89.10&89.92\\
% Our + VGG19& 63.04&82.33&87.04&66.16&
% 82.69&87.80&65.77&83.11&87.98&66.21&84.13&89.55
% \\
& VGG-19+ResNet-18 & 87.04 & 87.80& 87.98&89.55\\
&FedType&86.83&86.92&87.24&88.67\\\hline

\multirow{3}{*}{\textbf{CIFAR-100}} 
& Homo-VGG-19 & 65.91&67.52&69.81&69.98\\
   % Our + VGG19& 38.87&61.29&65.77&39.86&61.00&66.71&41.89&62.73&67.89&42.03&63.58&68.89\\
& VGG-19+ResNet-18 & 65.77&66.71&67.89&68.89\\
& FedType &65.69&65.45&67.07&67.35\\\hline

\multirow{2}{*}{\textbf{FedISIC-19}} 
& Homo-VGG-19 & 56.89 & 58.94 & 59.06 & 59.22\\
& VGG-19+ResNet-18 & 56.62&57.12&57.59&57.96\\
&FedType&55.95&56.86&56.68&57.21\\
\bottomrule 
\end{tabular}
}
\label{tab:app_largest}
\vspace{-0.1in}
\end{table*}

We can observe that the upper bound performance obtained by the Homo-VGG-19 model performs the best, and VGG-19+ResNet-18 is better than FedType but with marginal improvements, which aligns with our expectations. 
However, our model and VGG-19+ResNet-18 use ResNet-18 (with 11.17 million parameters) as the proxy model to exchange information between clients and the server. However, the Homo-VGG-19 model has 144 million parameters, which is 12.9X of our model. Taking the communication costs into consideration, the proposed FedType is an effective solution to address the model heterogeneity challenge in federated learning.





% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{Private models are all VGG-19 in our framework. FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc} 
% \toprule 
% &  \multicolumn{3}{c|}{\textbf{FedAvg}}&
% \multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ 
%    & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
%       \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
%       Our + VGG19& 83.98&89.67&91.35&86.20&
% 94.16&94.12&86.77&91.84&93.45&87.19&91.24&
% 94.33\\
%       Our &83.93&89.45&91.22&86.44&91.50
% &93.84&87.13&92.05&92.36&87.85&92.11
% &93.17
% \\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
% \midrule
% Our + VGG19& 63.04&82.33&87.04&66.16&
% 82.69&87.80&65.77&83.11&87.98&66.21&84.13&89.55
% \\
% Our&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
% 83.00&87.24&66.87&84.49&88.67\\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
%    Our + VGG19& 38.87&61.29&65.77&39.86&61.00&66.71&41.89&62.73&67.89&42.03&63.58&68.89\\
%    Our &38.17&
% 61.06&65.69&39.31&61.22&65.45&40.92&62.68&
% 67.07&41.24&62.96&67.35\\\hline
%    \multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
%    Our + VGG19& 43.21&53.26&56.62&43.56&53.89&57.12&42.98&
% 54.10&57.59&42.74&54.85&57.96\\
% Our&42.30&	53.48&	55.95&
% 41.77&	54.30&	56.86&
% 42.35&	53.85&	56.68&
% 41.82&	54.04&	57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_largest}
% \vspace{-0.1in}
% \end{table*}






% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{Homo private models are all VGG-19. We conduct the basic FL.FMNIST/CIFAR-10/CIFAR-100 datasets with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c} 
% \toprule 
% &  \multicolumn{1}{c|}{\textbf{FedAvg}}&
% \multicolumn{1}{c|}{\textbf{FedProx}} & \multicolumn{1}{c|}{\textbf{pFedMe}} & \multicolumn{1}{c}{\textbf{pFedBayes}}\\ \hline

%       \multicolumn{5}{c}{\textbf{FMNIST}} \\\hline
%       Homo VGG19 &92.86&94.05&94.26&94.87\\
%       Our &91.22
% &93.84&92.36&93.17
% \\\hline
%    \multicolumn{5}{c}{\textbf{CIFAR-10}} \\
% \midrule
% Homo VGG19&
% \\
% Our&86.83&86.92&87.24&88.67\\\hline
%    \multicolumn{5}{c}{\textbf{CIFAR-100}} \\\hline
%    Homo VGG19&\\
%    Our &65.69&65.45&67.07&67.35\\\hline
%    \multicolumn{5}{c}{\textbf{FedISIC-19}} \\\hline
%    Homo VGG19&56.89&58.94&59.06&59.22\\
% Our&55.95&
% 56.86&
% 56.68&
% 57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_largest_homo}
% \vspace{-0.1in}
% \end{table*}



\subsection*{W2 \& Q2}

We agree that training a shared global model with heterogeneous clients without introducing proxy models is one way to define model heterogeneity in federated learning. As discussed in W1, in this paper, we focus on the \textbf{personalized model heterogeneity} in federated learning, where each client maintains a fixed private model, but the structures of client models are not the same or even from the same global model. Thus, simply increasing the local model size cannot solve this issue since their model structures are different.

In our setting, we introduce a proxy model to make it possible to conduct the heterogeneous model aggregation. Our approach has several advantages: (1) Proxy models prevent the entire disclosure of the structure and parameters of private models, thereby bolstering privacy. (2) Typically, proxy models are much smaller than the private models maintained locally. This size difference means that transmitting proxy models between the server and clients can significantly reduce communication overhead in the FL framework.

\subsection*{W3}
In the current version, we only provide the empirical convergence analysis, which is detailed in Appendix G and illustrated in Figure 5. In future research, we intend to delve into the theoretical convergence analysis of the entire framework.


\subsection*{Follow-up question}
\textcolor{red}{\textit{Thank you for your response. I still have concerns about using the proxy model. For example, if the proxy model is ResNet-18, which has about 11M parameters, then why wouldn't the client directly use ResNet-50 as the local model (which has about 25M parameters) instead of two ResNet-18 models (one as the proxy model)? In my opinion, personalized models are required due to device heterogeneity, as some devices may have limited capacity to accommodate a large model. Thus, it is important to demonstrate that the use of the proxy model is more advantageous than simply increasing the local model size. Is there any experiment to demonstrate it? For example, could you compare FedType with FedAvg where all clients are using ResNet-50? I'd like to see how much benefit the clients with larger models in FedType can obtain and whether the clients with smaller models in FedType will have to make sacrifices or not. Since you are doing personalized federated learning, reporting average accuracy among the clients cannot provide enough insights to the benefit of each client.}}

Thank you for the prompt reply. We think you may misunderstand our setting. In our model heterogeneity setting, we assume that each client has its own model, and the client model structures among clients are different. These client models are \textbf{fixed} during the model training. This is a practical setting. For example, there are four institutions (c1, c2, c3, and c4) that want to enhance their private model performance but do not want to redeploy their current models (ResNet-18, ResNet-101, VGG-11, and VGG-19). A straightforward way is to introduce an identical proxy model, such as ResNet-18, as the mediator for information exchange.

The introduction of proxy models has three advantages. First, it enables the aggregation of client models even with heterogenous model structures. Second, the size of the proxy model is typically small compared to the private model, which will significantly save communication costs. Third, using the proxy models as the mediator, we do not need to upload any information regarding the private model and data. In such a way, it preserves the privacy.

As we mentioned before, in our setting, the client models are fixed and significantly different from each other. Thus, simply increasing the size of client models cannot solve the issue of heterogeneous model aggregation. For example, replacing ResNet-18+ResNet-18 with ResNet-50 and ResNet-34+ResNet-18 with ResNet-101 still faces the same issue -- the client model structures (i.e., ResNet-50 and ResNet-101) are different.



Adding a proxy model to each client does increase resource consumption. In fact, our design allows for flexible proxy model selection. As shown in Table 3, even using a smaller proxy model can still achieve the goal of heterogeneous model aggregation, but with a slight performance drop. We also discussed resource usage in Appendix M.

We can do the experiment to compare FedType with FedAvg, where all clients are using ResNet-50, but this would be unfair to our model FedType. As mentioned before, our model aims to solve the model structure heterogeneity issue in FL instead of the homogeneous setting. If we deploy two ResNet-18 models on all local clients and make them enhance each other with mutual learning, the personalized performance should be worse than the setting where all clients use ResNet-50. 

In fact, we have a similar experiment in Section 4.3, where we deploy all clients with the same model VGG-11 (132.86M) for the FedAvg baseline, and FedType uses ResNet-18 (11.17M) as the proxy model and VGG-11 as the private model. The total number of parameter sizes for each client is 144.03M. The results are shown in Figure 4. We can observe that the baseline performs slightly better than our approach, but the communication costs are significantly high. This experiment can confirm that our model can work for the homogeneous setting in an efficient way but with a slight performance drop. 

We hope our responses can solve your concerns. We are looking forward to further discussions. 


\newpage
\section*{Reviewer JJT3}

\subsection*{W1}
Thanks for pointing out the ablation analysis on the piece-wise calibration function $g()$. As suggested by the reviewer, we employ an increasing function $g()$ in the range [0,1], defined as $g = 0.5 \cdot \Delta^t + 0.5$, and $g = 0.5$ for $\Delta^t \in [-1, 0]$. 
We then carried out experiments on the CIFAR-10 dataset with $\alpha = 0.5$ to compare the new $g()$ function and the proposed one in Eq. (7). The results are reported in the subsequent table:

\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{New g() function. CIFAR-10 dataset with $\alpha = 0.5$}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\toprule 
&  \multicolumn{3}{c|}{\textbf{FedAvg}}&
\multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ \hline

   & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
    \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
    New g()&82.65&89.11&91.00&85.27&91.13&92.92
&86.06&91.58&92.25&86.45&91.89&93.08\\
    Ours &83.93&89.45&91.22&86.44&91.50
&93.84&87.13&92.05&92.36&87.85&92.11
&93.17\\\hline
   \multicolumn{13}{c}{\textbf{CIFAR-10}} \\\hline
   
   

New g()&61.04&80.26&83.11&63.43&81.79&84.60&
64.51&82.36&86.47&66.52&83.61&86.80\\
Ours &63.39&82.57&86.83&65.86&82.48&86.92&65.22&
83.00&87.24&66.87&84.49&88.67\\\hline
\multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
    New g()&35.5&58.31&62.45&37.88&58.93&63.22&37.69&60.14&66.85&41.11&61.64&66.57\\
    Ours&38.17&
61.06&65.69&39.31&61.22&65.45&40.92&62.68&
67.07&41.24&62.96&67.35\\\hline
\multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
New g()&36.7&44.14&50.62&36.81&46.65&53.52&
38.03&48.25&53.48&37.66&47.89&53.17\\
Ours &42.30&	53.48&	55.95&
41.77&	54.30&	56.86&
42.35&	53.85&	56.68&
41.82&	54.04&	57.21\\
\bottomrule 
\end{tabular}
}
\label{tab:app_new_g}
\vspace{-0.1in}
\end{table*}

We can observe that the performance will be significantly decreased if the new g() function is an increasing one. This further demonstrates the reasonable design of our calibration function.

\subsection*{W2}
Thanks for pointing it out. The results are calculated using the testing set. To avoid confusion, we will add specific descriptions in the updated version of the paper.

\subsection*{W3}



Thank you for posing this insightful question. The introduction of $\eta$ is to measure the prediction capability of the private and proxy models. A large $\eta$ indicates the behaviors of these two models are similar. However, there is no explicit relation between the change of $\eta$ and the convergence. As shown in Figure 6, the average value of $\eta$ has an overall increase trend but is unstable since it can achieve 1 at certain communication rounds. However, as shown in Figure 5, the average accuracy grows stably with increased communication rounds. Thus, the value of $\eta$ is not an indicator of the model convergence.

% We've illustrated the empirical convergence through Figure 5, which shows the progression of the value of $\eta$ across different communication rounds. By examining the interplay between the data in Figures 5 and 6, it is evident that $\eta$ increases as the system gradually approaches convergence through successive communication rounds. Moreover, once the system nears convergence, the value of $\eta$ stabilizes close to, or exactly at, 1. Given $\eta$'s role in quantifying the consensus level between the proxy and private models, its correlation with system convergence underscores the effectiveness and logical foundation of our approach. This alignment affirms the integrity of our design's impact on achieving consensus and system convergence.

\subsection*{W4}

Due to the space limit, we did such a comparison and listed the results in Appendix M. We assess computational efficiency by measuring training duration. Although our method slightly extends training time compared to the traditional symmetrical KD loss, this minor increase is counterbalanced by a noticeable enhancement in performance, as evidenced in the ablation study detailed in Section 4.2.3.

\newpage
\section*{Reviewer ytUi}


\subsection*{W1}
Thanks for pointing out this valuable comment. In our setting, clients hold different types of local models. Although several approaches focus on solving this challenging issue, they also need to use extra public data, as discussed in the Introduction and related work sections. For a fair comparison, we do not employ them as baselines since the proposed FedType is a public data-free method.

As the reviewer suggested, we conducted the following experiment on the CIFAR-100 dataset with $\alpha = 0.5$ by employing a representative heterogeneous model aggregation approach FedMD [1] as the baseline, where the public dataset used for training FedMD is CIFAR-10, and the number of public data is 5,000. The other settings are the same as the experiments demonstrated in Section 4.1. 

The average accuracy of FedMD is \textbf{65.82}, which is slightly better than the proposed FedType using FedAvg (65.69) and FedProx (65.45) as the aggregation method. However, it is worse than FedType with pFedMe (67.07) and pFedBayes (67.35). We can observe that our model FedType, even without using any extra public data but only employing advanced model aggregation techniques, can outperform existing approaches with additional data. This observation also further demonstrates the effectiveness of our model. Besides, our model does not exchange sensitive information to guarantee data privacy.

\textit{[1] Daliang Li and Junpu Wang. 2019. FedMD: Heterogenous federated learning via model distillation. NeurIPS 2019 Workshop on Federated Learning for Data Privacy and Confidentiality.}


% As highlighted by the reviewer, we discussed the landscape of heterogeneous federated learning in Section 2.1. The techniques outlined in the second paragraph necessitate the exchange of additional data, like class scores and label-wise representations, potentially elevating privacy risks. In contrast, our method requires only the sharing of proxy model parameters, steering clear of transmitting any client-sensitive information. Nevertheless, we would like to evaluate and contrast these methods in future studies, to ascertain their importance in achieving optimal performance, as recommended by the reviewer.

% As the reviewer suggested, we conducted the experiment of the baseline FedMD and FCCL. Both of them need to exchange extra information between the server and the clients and use public data. FedMD uses the labeled public data and FCCL uses the unlabeled public data. Following the setting in the paper FedMD, we use the CIFAR-10 as the public dataset and the CIFAR-100 as the private dataset. With maintaining all the other settings the same as our main paper, we report the results as follows

% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{Baselines on CIFAR-100 datasets with $\alpha = 0.5$}
% % \resizebox{1\textwidth}{!}
% {
% \begin{tabular}{c|c|c|c|c|c|c} 
% \toprule 
% Approach & Public Data &Extra Information&{\textbf{FedAvg}}&
% {\textbf{FedProx}} & {\textbf{pFedMe}} & {\textbf{pFedBayes}}\\ \hline



% FedType&No& No &65.69&65.45&67.07&67.35\\\hline
% FedMD&Yes&Yes& \multicolumn{4}{c}{65.82}\\



% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_baseline}
% \vspace{-0.1in}
% \end{table*}


\subsection*{W2}
We totally agree with the reviewer's comment. In our current experiments, we did not explore the relationship between the model architecture difference and the framework performance. To this end, we conducted the following experiment with $\alpha = 0.5$, and the other settings are the same as the main experiments shown in Table 1.

In this experiment, we fixed the proxy model, which is ResNet-18, but used different private models. 
\textbf{FedType-ResNet} denotes all the private client models selected from the ResNet family pool, including ResNet-18, ResNet-34, ResNet-50, RestNet-101, and ResNet 152. 
\textbf{FedType-VGG} denotes all the private models belonging to the VGG family, including VGG-11, VGG-13, VGG-16, and VGG-19.
\textbf{FedType-Mix} is our model used in the main experiments, which uses the mixed ResNet and VGG client models.
We report the results in the following table.

% Thanks for the reviewer's constructive suggestion. In our current experiments, we used ResNet-18 as the proxy model, and the local private models cover ResNet-18, ResNet-34, ResNet-50, RestNet-101, ResNet 152, VGG-11, VGG-13,
% VGG-16, and VGG-19. To explore the influence of proxy model selection, we list the results of different types of private models obtained by running FedType with FedAvg on CIFAR-10 ($alpha = 0.5$)in the following table:

% \begin{table*}[!h]
% \centering
%     \begin{tabular}{c|c|c||c|c|c}
%     \hline
%     Model Type & Model Size & Avg. Accuracy &  Model Type & Model Size & Avg. Accuracy\\\hline
%       ResNet-18   & 11.17 M& & VGG-11 & 132.86 M& \\
%       ResNet-34   & 21.29 M& & VGG-13 &133.05 M &\\
%       ResNet-50   & 23.53 M& & VGG-16 &138.36 M & \\
%       RestNet-101 & 42.50 M& & VGG-19 &143.67 M &\\ 
%       ResNet 152 & 58.16 M & & & &\\ \hline
%       \textbf{ResNet Avg.} & & & \textbf{VGG Avg.} & &\\\hline

%     \end{tabular}
% \end{table*}

% We can observe that \textcolor{red}{XXX}

% Inspired by the reviewer's comment, we also conducted the following experiment with $\alpha = 0.5$ to explore the relationships between the proxy and private model selection. 





\begin{table*}[!h]
\centering
\vspace{-0.1in}
\caption{All the clients' personal models are from ResNet family models or the VGG family models.  FMNIST/CIFAR-10/CIFAR-100 with $\alpha = 0.5$/Fed-ISIC dataset}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\toprule 
&  \multicolumn{3}{c|}{\textbf{FedAvg}}&
\multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\\hline 
   & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
    \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
    FedType-ResNet&84.55&89.63&91.12&85.51&91.86&93.61&87.41
&93.55&93.64&87.62&92.33&94.86\\
    FedType-Mix  &83.93&89.45&91.22&86.44&91.50
&93.84&87.13&92.05&92.36&87.85&92.11
&93.17\\
    FedType-VGG&83.22&88.87&90.86&84.31&91.07&92.46
&86.65&91.77&92.20&87.04&91.98&92.46\\\hline

   \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
\hline

FedType-ResNet&64.59&83.62&86.88&66.11&83.79&87.25&66.89&84.08&87.10&67.03&
84.55&88.96\\
FedType-Mix&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
83.00&87.24&66.87&84.49&88.67\\
FedType-VGG&61.22&80.61&83.07&64.95&80.87&84.14
&63.40&81.36&84.52&65.48&81.27&86.11\\\hline

\multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline

    FedType-ResNet&38.95&62.48&65.53&40.66&63.07&
67.89&41.56&62.97&68.16&41.82&63.57&67.94\\
    FedType-Mix&38.17&
61.06&65.69&39.31&61.22&65.45&40.92&62.68&
67.07&41.24&62.96&67.35\\
FedType-VGG&35.96&58.74&62.41&36.77&58.91&62.88
&39.52&59.61&63.05&40.08&61.63&63.85\\\hline

\multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline

FedType-ResNet&42.86&53.55&55.84&42.84&
55.51&56.90&42.21&53.88&57.03&42.37&55.22&
57.10\\
FedType-Mix&42.30&	53.48&	55.95&
41.77&	54.30&	56.86&
42.35&	53.85&	56.68&
41.82&	54.04&	57.21\\
FedType-VGG&40.76&51.06&52.90&42.04&51.98&53.69
&42.13&52.61&53.12&41.01&52.48&54.55\\
\bottomrule 
\end{tabular}
}
\label{tab:app_resnet}
\vspace{-0.1in}
\end{table*}


We have several exciting observations. First, the private model performs better than the proxy model, which is better than the global model. This observation is the same as what we discussed in the main results. Second, FedType-ResNet outperforms FedType-Mix, which further outperforms FedType-VGG. This observation demonstrates that if the proxy model and the private models have similar model architectures, the proposed bidirectional knowledge distillation performs the best. These experimental results confirm the reviewer's statement. We will add these results to the final version.






% Based on the findings, it is evident that performance metrics, when using ResNet or VGG model families, tend to be superior or inferior compared to our initially reported outcomes. This observation corroborates the reviewer's insights regarding performance enhancements or declines resulting from the model's architectural congruence with KD techniques. These outcomes further validate the robustness and adaptability of our proposed framework across diverse conditions.









% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{Proxy model 18, stats on CIFAR-10 dataset with $\alpha = 0.5$}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|cccccc|ccc} 
% \toprule 
%    & ResNet-18 & ResNet-34 &ResNet-50  & ResNet-101 & ResNet-152 &VGG-11& VGG-13 & VGG-16 &VGG-19 \\\hline
%    Parameter Sum\\
%    Client-level Avg ACC\\
%    Model-level Avg ACC\\
   
%     % \multicolumn{13}{c}{\textbf{FMNIST}} \\

% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_new_proxy model}
% \vspace{-0.1in}
% \end{table*}
























% \begin{table*}[!h]
% \centering
% \vspace{-0.1in}
% \caption{All the clients' personal models are from VGG family models.  FMNIST/CIFAR-10/CIFAR-100 with $\alpha = 0.5$/Fed-ISIC dataset}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|ccc|ccc} 
% \toprule 
% &  \multicolumn{3}{c|}{\textbf{FedAvg}}&
% \multicolumn{3}{c|}{\textbf{FedProx}} & \multicolumn{3}{c|}{\textbf{pFedMe}} & \multicolumn{3}{c}{\textbf{pFedBayes}}\\ 
%    & global & proxy &private  & global & proxy &private& global & proxy &private & global & proxy &private\\\hline
%     \multicolumn{13}{c}{\textbf{FMNIST}} \\\hline
%     FedType (VGG)&84.55&89.63&91.12&85.51&91.86&93.61&87.41
% &93.55&93.64&87.62&92.33&94.86\\
%     FedType  &83.93&89.45&91.22&86.44&91.50
% &93.84&87.13&92.05&92.36&87.85&92.11
% &93.17\\\hline
%    \multicolumn{13}{c}{\textbf{CIFAR-10}} \\
% \hline
% FedType (VGG)&64.59&83.62&86.88&66.11&83.79&87.25&66.89&84.08&87.10&67.03&
% 84.55&88.96\\
% FedType&63.39&82.57&86.83&65.86&82.48&86.92&65.22&
% 83.00&87.24&66.87&84.49&88.67\\\hline
% \multicolumn{13}{c}{\textbf{CIFAR-100}} \\\hline
%     FedType (VGG)\\
%     FedType&38.17&
% 61.06&65.69&39.31&61.22&65.45&40.92&62.68&
% 67.07&41.24&62.96&67.35\\\hline
% \multicolumn{13}{c}{\textbf{FedISIC-19}} \\\hline
% FedType(VGG)&42.86&53.55&55.84&42.84&
% 55.51&56.90&42.21&53.88&57.03&42.37&55.22&
% 57.10\\
% FedType&42.30&	53.48&	55.95&
% 41.77&	54.30&	56.86&
% 42.35&	53.85&	56.68&
% 41.82&	54.04&	57.21\\
% \bottomrule 
% \end{tabular}
% }
% \label{tab:app_vgg}
% \vspace{-0.1in}
% \end{table*}


\subsection*{Questions}
Thanks for pointing out the typo. We will fix it in the final version.
% We apologize for the typos. You are correct. Figure 4.3 should be Figure and FedERAL should be FedType. We will fix the typos in the updated version of the paper.

\subsection*{Limitations}
The proposed framework has two major limitations. First, as discussed in W2, selecting the proxy model is non-trivial and further influences the framework performance. In future work, we plan to design an automatic strategy to adaptively select the proxy model according to the types of private models. Second, although the proposed framework is effective and efficient, the designed uncertainty-based asymmetrical reciprocity learning between the proxy and private model runs slightly slower than the naive bidirectional knowledge distillation. Thus, we need to develop a more efficient approach to accelerate this step. From our perspective, there is no negative social impact on the designed framework.


\newpage
\section*{Reviewer i2GH}

\subsection*{Q1}
We totally agree with the reviewer's comment that basic mutual learning is not a novel technique. However, existing work such as FML only uses hyperparameter weights to control the proportion of knowledge transfer, which may not be accurate. In this paper, our goal is to design a novel uncertainty-based asymmetrical reciprocity learning to address this problem. As the reviewer pointed out, this is our main contribution.

\subsection*{Q2}
Thanks for pointing out the existing work. In fact, in our ablation study (Sec 4.2.3), we employed a mutual learning baseline, FedType\_sym, which is a specific version of FML with $\alpha = \beta = 0.5$. FedProto, without using public data, also focuses on heterogeneous model aggregation, but it uses the class prototype as the proxy information. Such information is obtained directly from client data, which may have privacy concerns. Besides, a 1-D prototype vector may have enough knowledge to represent the knowledge of client models. Thus, it is hard to guarantee the performance, which can be found in the table in Q3. We will add these approaches and discussions to the related work section in the final version. 


% We totally agree with the reviewer that the basic mutual learning in FL has been developed. In our designed approach, we designed a novel uncertainty-based asymmetrical reciprocity learning to conduct the bi-directional learning, which considers the model size and the information diversity they carry. In our ablation study (Sec 4.2.3), FedType\_sym can be treated as a traditional mutual learning setting and our approach shows superior performance over it on the CIFAR-10 and Fed-ISIC 19 datasets in Table 2. 

% \subsection*{Q2}
% Thanks for pointing out. We will add them to our related work section in our updated version paper.

\subsection*{Q3}
We express our gratitude for the insightful feedback provided by the reviewer. The referenced baseline, FML, has been evaluated alongside our methodology in the ablation study within the context of FedType\_sym, where we implement a conventional knowledge distillation process. We intend to incorporate additional notes in the updated version of our paper to clarify this comparison further.

As mentioned in Q2, we validated a particular version of FML, which is FedType\_sym, in our ablation study (Sec 4.2.3). Besides, we added FedProto as a baseline, where $\lambda = 1$. Here, we show the results on the CIFAR-10 and Fed-ISIC19 datasets in the following table, where the settings are the same as those demonstrated in Sec 4.2.3.
\begin{table*}[h]
    \centering
    \begin{tabular}{c|c|c}
    \hline
        Dataset &  CIFAR-10 & Fed-ISIC19 \\\hline
         FML (FedType\_sym)& 82.24 & 49.89 \\
         FedProto & 78.17 & 42.60 \\
         FedType & 86.83 & 55.95 \\\hline
    \end{tabular}
    \caption{Extra baselines}
    \label{tab:my_label}
\end{table*}

In Sec. 4.2.3, we had compared FML (FedType\_sym) with FedType. In this experiment, we mainly analyze the new baseline FedProto, which takes the class prototype as the proxy information. As discussed in Q2, the 1-D prototype vector does not have enough capability to represent the characteristics of client data. Thus, FedProto performs the worst. However, in our setting, the large number of proxy model parameters contains sufficient information. Besides, uploading prototype vectors directly obtained from client data may have privacy concerns. However, our model neither uploads any data-related information nor private model parameters, which is another advantage of our model design.
We really appreciate the reviewer's invaluable comment, which significantly improves the quality of our experiments. We will add the results of these two baselines in the main results in Table 1 in the final version. 

\subsection*{Q4}

Thanks for the reviewer's suggestion. We provided the results of the \textbf{communication cost} reduction in Sec 4.3 and Figure 4. Compared with exchanging the clients' private model parameters, our approach only transmits around 8\% of baselines' parameters while maintaining comparable performance. As for the \textbf{computational cost}, due to the page limit, we put the quantitative results in Appendix M using the training time compared with different training losses. The results demonstrated that our approach is able to boost the performance with a limited extra computational time.  In line with the reviewer's advice, we aim to decrease the computational cost further in our subsequent research efforts.



